Learning Hierarchical Polynomials of Multiple Nonlinear Features with Three-Layer Networks

In deep learning theory, a critical question is to understand how neural networks learn hierarchical features. In this work, we study the learning of hierarchical polynomials of \textit{multiple nonlinear features} using three-layer neural networks. We examine a broad class of functions of the form $f^{\star}=g^{\star}\circ \bp$, where $\bp:\mathbb{R}^{d} \rightarrow \mathbb{R}^{r}$ represents multiple quadratic features with $r \ll d$ and $g^{\star}:\mathbb{R}^{r}\rightarrow \mathbb{R}$ is a polynomial of degree $p$. This can be viewed as a nonlinear generalization of the multi-index model \citep{damian2022neural}, and also an expansion upon previous work that focused only on a single nonlinear feature, i.e. $r = 1$ \citep{nichani2023provable,wang2023learning}. Our primary contribution shows that a three-layer neural network trained via layerwise gradient descent suffices for \begin{itemize}\item complete recovery of the space spanned by the nonlinear features \item efficient learning of the target function $f^{\star}=g^{\star}\circ \bp$ or transfer learning of $f=g\circ \bp$ with a different link function \end{itemize} within $\widetilde{\cO}(d^4)$ samples and polynomial time. For such hierarchical targets, our result substantially improves the sample complexity ${\Theta}(d^{2p})$ of the kernel methods, demonstrating the power of efficient feature learning. It is important to highlight that{ our results leverage novel techniques and thus manage to go beyond all prior settings} such as single-index and multi-index models as well as models depending just on one nonlinear feature, contributing to a more comprehensive understanding of feature learning in deep learning.

==> deprecated/deprecated.tex <==
\paragraph*{Simplified Learner Networks.}
\[
f_{\theta}(\bx):=\sum_{i=1}^{m}a_{i}\sigma\left(\langle W_i,\bx\bx^{\top} \rangle+b_i\right)
\]
After first-step gradient w.r.t. $W$, $W$ becomes $T(W)$, which is written as
\begin{align*}
    T(W)\sim \EE_{x}\left[f(\bx)\langle W,\bx\bx^{\top} \rangle \bx\bx^{\top}\right]
\end{align*}
(omit constants and high order terms\zh{check})
$T(W)$ is a linear operator, we aim to show that:
\begin{itemize}
    \item $T(A_i)=\sum_{j=1}^{r}\lambda_{i,j}A_j+B_i$. $i\in[r]$ here $\norm{B_i}{F}= o_d(1)$ and $[\lambda_{i,j}]$ is non-degenerate.
    \item $T(B)=B'$ for $\norm{B}{F}=1$ and $B\perp A_i$, $\forall i \in [r]$, here $\norm{B'}{F}= o_d(1)$
\end{itemize}
Thus, we can decompose $T$ into $T=T^{\star}+T^{\prime}$, where $T^{\star}$ maps $A_i$ to $\sum_{j=1}^{r}\lambda_{i,j}A_j$  and $B$ to $\mathbf{0}^{d\times d}$ and $\norm{T^{\prime}(W)}{op}\le o_d(1)$ for any $\norm{W}{F}\le 1$.
Then we consider infinite-width random feature case and find $a(W)$ and $b(W)$ with small $L_2$ norm (constant-size?)\zh{$b$ cannot be trained}such that
\begin{align}\label{equ:: infinite width RF}
   f(\bx)=\EE_{W}\left[a(W)\sigma\left(\langle \bT^{\star}(W),\bx\bx^{\top}\rangle+b(W)\right) \right]. 
\end{align}

Then we compute the difference between \eqref{equ:: infinite width RF} and 
\[
g(\bx)=\EE_{W}\left[a(W)\sigma\left(\langle T(W),\bx\bx^{\top}\rangle+b(W)\right) \right].
\]
Using the regularity of $\sigma$ and the bounded operator norm of $T'(W)$ as well as the bounded $L_2$ norm of $a(W)$, the difference should be $o_{d}(1)$.
\begin{assumption}\label{assump::basic assump}
    For the target function $g:\RR^{r}\rightarrow \RR$, we assume $g(\cdot)$ is $L-$Lipschitz. Moreover, we assume $\EE_{\bz \sim \cN(\bzero_r,I_r)}\left[{g(\bz)}\right]=0$~ and ~$\EE_{\bz \sim \cN(0,I_r)}\left[{\nabla g(\bz)}\right]=\bzero_r$. The features $\bA_1$, $A_2$, $\dots$, $\bA_r$ are orthogonal matrices satsifying $\EE\brac{\bx^{\top}A_i\bx}=0$~ and ~$\EE\brac{\paren{\bx^{\top}A_i\bx}^2}=1$, for $i=1,2,\dots,r$. This implies that $\tr(A_i)=0$ and $\norm{A_i}{F}={1}/{\sqrt{2}}$. Moreover, we assume $\norm{A_i}{op}=\cO(1/\sqrt{d})$.
\end{assumption}

\begin{proof}[Original proof of Lemma \ref{lemma::AiB strong}]
    Let $\tau > 1/\sqrt{d}$ be a threshold to be determined later. Decompose $B$ as follows:
    \begin{align*}
        B = \sum_{j=1}^d \lambda_j \bu_j\bu_j^{\top} = \sum_{\abs{\lambda_j} > \tau} \lambda_j \left(u_j u_j^{\top} - \frac{1}{d}\bI\right) - \sum_{k=1}^{r}\frac{1}{\norm{\bA_k}{F}^2} \sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j \cdot \bA_k + \tilde \bB,
    \end{align*}
    where $\set{u_j}_{i=1}^{d}$ are orthogonal unit vectors and
    \begin{align*}
        \tilde \bB = \sum_{\abs{\lambda_j} \le \tau} \lambda_j\bu_j\bu_j^{\top} + \bI \cdot \frac{1}{d}\sum_{\abs{\lambda_j} > \tau}\lambda_j + \sum_{k=1}^{r}\frac{1}{\norm{\bA_k}{F}^2} \sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j \cdot \bA_k.
    \end{align*}
    By construction, we have
    \begin{align*}
        \tr(\tilde \bB) = \sum_{\abs{\lambda_j} \le \tau} \lambda_j + \sum_{\abs{\lambda_j} > \tau}\lambda_j = \sum_{j \in [d]} \lambda_j = 0.
    \end{align*}
    Moreover, for any $k \in[r]$, we have
    \begin{align*}
        \langle \tilde \bB, \bA_k \rangle = \sum_{\abs{\lambda_j} \le \tau} \lambda_j \bu_j^{\top}\bA_k\bu_j + \sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j = \langle \bA_k, B \rangle = 0.
    \end{align*}
    Therefore by \Cref{lemma::AiB weak},  we have
    \begin{align}\label{equ::bound tilde B}
\abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\langle \bA_i,\bx\bx^{\top}\rangle \langle \tilde \bB,\bx\bx^{\top}\rangle}} \lesssim \paren{\frac{r}{\sqrt{d}}+\frac{\norm{\tilde \bB}{op}}{\norm{\tilde \bB}{F}}}\norm{\tilde \bB}{F}Lr\log^2 d
    \end{align}
    Since $\sum_{j=1}^{d}\lambda^2_j=1/2$,  there are at most $O(\tau^{-2})$ indices $j$ satisfying $\abs{\lambda_j} > \tau$, which gives rise to
    \begin{align*}
        \sum_{\abs{\lambda_j} > \tau}\abs{\lambda_j} \lesssim \sqrt{\tau^{-2} \cdot \sum_{\abs{\lambda_j} > \tau}\abs{\lambda_j}^2} \le \tau^{-1}.
    \end{align*}
    Thus, we can bound the Frobenius norm of $\tilde \bB$ by
    \begin{align*}
        \norm{\tilde \bB}{F}^2 &\lesssim \sum_{\abs{\lambda_j}\le \tau}\lambda_j^2 + \frac{1}{d}\left(\sum_{\lambda_j > \tau}\lambda_j\right)^2 + \norm{\sum_{k=1}^{r}\frac{1}{\norm{\bA_k}{F}^2}\sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j\cdot \bA_k}{F}^2\\
        &= \norm{\tilde \bB}{F}^2 \sum_{\abs{\lambda_j}\le \tau}\lambda_j^2 + \frac{1}{d}\left(\sum_{\lambda_j > \tau}\lambda_j\right)^2 + \sum_{k=1}^{r}\frac{1}{\norm{\bA_k}{F}^2}\abs{\sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j}^2 \\
        &\lesssim  \sum_{\abs{\lambda_j}\le \tau}\lambda_j^2 +\left(\frac{1}{d}+\sum_{k=1}^{r}\norm{\bA_k}{op}^2\right) \abs{\sum_{\abs{\lambda_j} > \tau} \lambda_j}^2\\
        &\lesssim 1 + \frac{r}{d\tau^2}\\
        &\lesssim r.
    \end{align*}
    and
    \begin{align*}
        \norm{\tilde \bB}{op} &\le \tau + \left(\frac{1}{d} + \sum_{k=1}^r\norm{A}{op}\right)\abs{\sum_{\abs{\lambda_j} > \tau}\lambda_ju_j^{\top}Au_j}\\
        &\lesssim \tau + \frac{r}{d\tau}.
    \end{align*}

    Thus, plugging the norm bounds into \eqref{equ::bound tilde B}, we obtain that
    \begin{align*}
    \abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\langle \bA_i,\bx\bx^{\top}\rangle \langle \tilde \bB,\bx\bx^{\top}\rangle}} 
    \lesssim \left(\frac{r^{3/2}}{\sqrt{d}} +\tau + \frac{r}{d\tau}\right)Lr \log^2 d.
    \end{align*}
    
    Next, applying Lemma \ref{lemma::Ai u}  with $u=u_1$, $u_2$, $\dots$, $u_d$ and $\mathbf{1}_d/\sqrt{d}$, we have
    \begin{align*}    \abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\left\langle \bA_i,\bx\bx^{\top}\right\rangle(\bu_j^{\top}\bx)^2}} \lesssim \frac{Lr^2 \log^2 d}{\sqrt{d}},~~~\forall j \in[d]
    \end{align*}
    and
    \begin{align*}
        \abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\left\langle \bA_i,\bx\bx^{\top}\right\rangle\frac{\norm{x}{2}^2}{d}}} \lesssim \frac{Lr^2 \log^2 d}{\sqrt{d}}.
    \end{align*}
    Thus, we have
    \begin{align*}
&\quad \abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\left\langle A_i,\bx\bx^{\top}\right\rangle \left\langle  \sum_{\abs{\lambda_j} > \tau}\lambda_j\left(\bu_j\bu_j^{\top} - \frac{1}{d}\bI\right),\bx\bx^{\top}\right\rangle}} \\
         &\le \sum_{\abs{\lambda_j} > \tau}\abs{\lambda_j}\frac{Lr^2 \log^2 d}{\sqrt{d}}\\
        &\lesssim \frac{Lr^2 \log^2 d}{\sqrt{d}\tau}.
    \end{align*}

    Moreover, by Lemma \ref{lemma::Ai Aj}, we have
    \begin{align*}
    &\quad \abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\left\langle A_i,\bx\bx^{\top}\right\rangle \left\langle \sum_{k=1}^{r}\frac{1}{\norm{\bA_k}{F}^2} \sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j \cdot \bA_k ,\bx\bx^{\top}\right\rangle}}\\
    &\lesssim \sum_{k=1}^{r}\abs{\sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j} \left(\EE_{\bz \sim \cN(\bzero_r,\bI_r)}\brac{\nabla^2 g(\bz)}_{k,i} +\frac{Lr^2 \log^2 d}{\sqrt{d}} \right)\\
    &\lesssim \sum_{k=1}^{r} L\abs{\sum_{\abs{\lambda_j} > \tau}\lambda_j \bu_j^{\top}\bA_k\bu_j} \\ &\lesssim \frac{Lr}{\sqrt{d}\tau}.
    \end{align*}
    
    Altogether, we have
    \begin{align*}
&\quad\abs{\EE\brac{g(\bx^{\top}\bA_1\bx,\dots,\bx^{\top}\bA_r\bx)\langle A_i,\bx\bx^{\top}\rangle \langle B,\bx\bx^{\top}\rangle}}\\
        &\lesssim \left(\frac{r^{3/2}}{\sqrt{d}} +\tau + \frac{r}{d\tau}\right)Lr \log^2 d+ \frac{Lr^2 \log^2 d}{\sqrt{d}\tau}+ \frac{Lr}{\sqrt{d}\tau}\\
        &\lesssim d^{-1/4}Lr^2\log^2 d. 
    \end{align*}
    where we set $\tau = d^{-1/4}$. The proof is complete.
\end{proof}

For simplicity, we vectorize $W$ as $\bw=\text{vec}(W)\in \RR^{d^2}$, and we similarly define $\ba_1,\ba_2,\dots,\ba_r$ as the flattened vector of $\bA_1,A_2,\dots,\bA_r$. Then the linear operator $T^{\star}$ can be expressed as the following matrix
\begin{align*}
    \bT^{\star}=\sqrt{2}\bA^{\top}H\bA \in \RR^{d^2 \times d^2},~~~\text{where}~~~\bA=[\ba_1,\ba_2,\dots,\ba_r]^{\top} \in \RR^{r\times d^2}.
\end{align*}
Denote $\Pi$ the orthogonal projection onto $\text{span}(\ba_1,\ba_2,\dots,\ba_r)$. We define the finite-sample version of $T$ as $T_n$, which is defined as
\begin{align*}
    T_n(W)=\frac{1}{n}\sum_{i=1}^{n}f(x_i)\langle W,x_ix_i^{\top} \rangle x_ix_i^{\top}.
\end{align*}


and denote $r_n=T_n-T$ and $r_{\star}=T-T^{\star}$. Here $r_{\star}$ can be seen as a symmetric $d^2 \times d^2$ matrix. Then from the lemmas above we know $\norm{r_{\star}}{op}\lesssim d^{-1/4}Lr^{5/2}\log^2 d$. From basic concentration theory we know  $\norm{r_n(\bw)}{2}\lesssim {d}/{\sqrt{n}}$ with high probability \hengyu{uncertain, the standard error of $\norm{f(\bx)\langle \bx\bx^{\top},W \rangle \bx\bx^{\top}}{F}$ scales as $d?$}\zh{concentration should not be hard I guess}

Now we try to replicate the results of Appendix A.2.2 in Alex's paper. We first prove that
\begin{align*}
    \text{Mat}\paren{\EE\brac{\paren{\Pi T_n(\bw)}^{\otimes 2k}}} \succsim \Pi_{\text{sym}},
\end{align*}
where the expectation is taken w.r.t. $\bw \sim \cN(\bzero,\bI_{d^2}/d^2)$. 
It suffices to prove that for any symmetric ($r$-rank) $k$-tensor $K$\hengyu {Alex verifies for all, but I think $r-$rank is enough?} with $\norm{K}{F}=1$, we have
\begin{align*}
    \EE\brac{\paren{\Pi T_n(\bw)}^{\otimes 2k}}(K,K) \gtrsim \frac{\lambda_{\min}(H)^4}{d^4}.
\end{align*}
Note that 
\begin{align*}
    \left\langle K, \paren{\Pi T_n(\bw)}^{\otimes k} \right\rangle = \left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle +\delta(\bw),
\end{align*}
where 
\begin{align*}
    \abs{\delta(\bw)}&\lesssim \sum_{i=1}^{k} \abs{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i} \otimes \paren{(r_n+r_{\star})(\bw)}^{\otimes i}} }
\end{align*}


By Young's inequality, we have
\begin{align}
    \EE\brac{\left\langle K, \paren{\Pi T_n(\bw)}^{\otimes k} \right\rangle^2} \geq \EE\brac{\frac{1}{2}\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2}-\EE\brac{\delta(\bw)^2} \label{equ::lower bound T}
\end{align}

\textbf{First attempt: following Alex's proof:}

Note that
\begin{align*}
    \abs{\delta(\bw)}\lesssim \sum_{i=1}^{k}\norm{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i}} }{F}\paren{\norm{\Pi r_n(\bw)}{2}
+\norm{\Pi r_{\star}(\bw)}{2}}^{i}.
\end{align*}

Now, by Cauchy-Schwarz inequality, we can bound $\delta(\bw)$ by
\begin{align}
    \EE\brac{\delta(\bw)^2}&\lesssim \sum_{i=1}^{k}\sqrt{\EE\brac{\norm{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i}} }{F}^4} \EE\brac{\paren{\norm{\Pi r_n(\bw)}{2}
+\norm{\Pi r_{\star}(\bw)}{2}}^{4i}}} \nonumber\\
&\lesssim \sum_{i=1}^{k}\EE\brac{\norm{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i}} }{F}^2} \sqrt{\EE\brac{\paren{\norm{\Pi r_n(\bw)}{2}
+\norm{\Pi r_{\star}(\bw)}{2}}^{4i}}} \label{equ::delta bound}
\end{align}
The last inequality follows from the fact that $ \norm{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i}} }{F}^2$ are polynomials of Gaussian. Let $\tilde K$ be another symmetric $r$-rank  $k$-tensor defined by $$\tilde K(\bw_1,\bw_2,\dots,\bw_k)=K(\bT^{\star}\bw_1,\bT^{\star}\bw_2,\dots,\bT^{\star}\bw_k).$$ By Corollary 8 in Alex's paper, we have
\begin{align*}
    \EE\brac{\norm{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i}} }{F}^2} &\le \frac{1}{\lambda_{\min}(\bT^{\star})^{2i}}\EE\brac{\norm{\tilde K(\bw^{\otimes k-i})}{}^2}\\
    &\lesssim \frac{d^{2i}}{\lambda_{\min}(\bT^{\star})^{2i}}\EE\brac{\tilde K(\bw^{\otimes k})^2} \\
    &=\frac{d^{2i}}{\lambda_{\min}(\bT^{\star})^{2i}} \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2}.
\end{align*}\hengyu{This step is not tight, because we do not use the r-rank, try to use colo 9}
Plugging into \eqref{equ::delta bound} gives rise to
\begin{align*}
    \EE\brac{\delta(\bw)^2}&\lesssim \sum_{i=1}^{k}\frac{1}{\lambda_{\min}(\bT^{\star})^{2i}} \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2}\sqrt{\EE\brac{\paren{\norm{\Pi r_n(\bw)}{2}
+\norm{\Pi r_{\star}(\bw)}{2}}^{4i}}}  \\
    &\lesssim \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2} \sum_{i=1}^{k} \paren{\frac{{d^2}/{\sqrt{n}}+d\cdot d^{-1/4}Lr^{5/2}\log^2 d}{\lambda_{\min}(\bT^{\star})}}^{2i}.
\end{align*}
\hengyu{This step does not utilize the projection $\Pi$. I wonder if we can prove $\EE\brac{\norm{\Pi \br_{\star}(\bw)}{}^2}\lesssim r/{d^2}\cdot \norm{\br_\star}{op}^2$}
It seems difficult to control $\delta(\bw)$.

\textbf{A second attempt: simple case of $k=2$:}

When $k=2$, we just write $K$ as a symmetric $d^{2}\times d^{2}$ matrix, and we can expand $\delta(\bw)$ as
\begin{align*}
    \delta(\bw)=2\langle K, (T^{\star}\bw)\otimes \br (\bw) \rangle + \langle K, \br (\bw)^{\otimes 2} \rangle,
\end{align*}
where $\br=\br_n+\br_{\star}$.
Since
\begin{align*}
    \EE\brac{\langle K, (T^{\star}\bw)\otimes \br_{\star} (\bw) \rangle^2}=&\frac{1}{d^4} \paren{\tr\paren{\br_{\star} K\bT^{\star}}^2 +2 \tr\paren{\paren{\br_{\star} KT^{\star}}^2}}\\
    &\le \frac{1}{d^4}\paren{\norm{\br_{\star} K}{F}^2\norm{\bT^{\star}}{F}^2+2\norm{\br_{\star} K\bT^{\star}}{F}^2}\\
    &\le \frac{1}{d^4}\paren{\norm{\br_{\star}}{op}^2\norm{\bT^{\star}}{F}^2+2\norm{\br_{\star}}{op}^2\norm{\bT^{\star}}{op}^2}\\
    &= \frac{\norm{\br_{\star}}{op}^2}{d^4}\paren{\norm{\bT^{\star}}{F}^2+\norm{\bT^{\star}}{op}^2},
\end{align*}
and similarly we have
\begin{align*}
    \EE\brac{\langle K,  \br_{\star} (\bw)^{\otimes 2} \rangle^2}=&\frac{1}{d^4} \paren{\tr\paren{\br_{\star} K \br_{\star}}^2 +2 \tr\paren{\paren{\br_{\star} K \br_{\star}}^2}}\\
    &\le \frac{1}{d^4} \paren{\tr\paren{\br_{\star} \sum_{i=1}^{r}\lambda_i \ba_i\ba_i^{\top} \br_{\star} }+2 \tr\paren{\paren{\br_{\star} K \br_{\star}}^2}} \\
    &\le \frac{1}{d^4}\paren{\paren{\sum_{i=1}^{r}\lambda_i\norm{\br_{\star} \ba_i}{2}^2  }^2+2 \norm{r}{op}^4} \\
    & \le \frac{1}{d^4}\paren{\paren{\sum_{i=1}^{r}\lambda_i\norm{\br_{\star}}{op}^2  }^2+2 \norm{r}{op}^4} \\
    & \le \frac{1}{d^4} \paren{(r+2)\norm{\br_{\star}}{op}^4  }. 
\end{align*}
Moreover, we suppose that with high probability, 
\begin{align*}
    \norm{\br_{n}(\bw)}{2} \lesssim \frac{d}{\sqrt{n}},
\end{align*}
so we have
\begin{align*}
    \EE\brac{\langle K, (\bT^{\star}\bw)\otimes \br_{n} (\bw) \rangle^2}&\le \EE\brac{\norm{K\bT^{\star}\bw}{}^2 \norm{\br_n(\bw)}{}^2}\\
    &\lesssim \frac{\norm{K\bT^{\star}}{F}^2}{d^2}\frac{d^2}{n}\\
    &\le \frac{\lambda_{\max}(H)^2r}{n} \cdot 
\end{align*}
Moreover, 
\begin{align*}
    \EE\brac{\langle K,  \br_{n} (\bw)^{\otimes 2} \rangle^2}&\le \EE\brac{\norm{K}{F}^2 \norm{\br_n(\bw)}{}^4}\\
    &\lesssim \frac{d^4}{n^2}.
\end{align*}
Thus, we have
\begin{align*}
    \EE\brac{\delta(\bw)^2} \lesssim \frac{\norm{\br_{\star}}{op}^2}{d^4}\paren{\norm{\bT^{\star}}{F}^2+\norm{\bT^{\star}}{op}^2} + \frac{r\norm{\br_{\star}}{op}^4}{d^4}+ \frac{\lambda_{\max}(H)^2}{n}+\frac{d^4}{n^2}.
\end{align*}

On the other hand, 
\begin{align*}
    \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes 2} \right\rangle^2}&=\frac{1}{d^4} \paren{\tr\paren{\bT^{\star} K \bT^{\star}}^2 +2 \tr\paren{\paren{\bT^{\star} K \bT^{\star}}^2}} \\
    & \gtrsim \frac{\lambda_{\min}(\bT^{\star})^4}{d^4}\\
    &\geq  \frac{\lambda_{\min}(H)^4}{d^4} .
\end{align*}
\hengyu{This step should use the fact $K$ lies in the span of $\bT^{\star}$}
Thus, we only need to choose $n=Cd^4\lambda_{\max}(H)^2/\lambda_{\min}(H)^4 \text{poly}(r)$ and $d=\text{poly}(r)$ \hengyu{not sure about the degree} so that $\norm{\br_{\star}}{op}^2$ is small enough to ensure 
\begin{align*}
    \EE\brac{\paren{\Pi T_n(\bw)}^{\otimes 4}}(K,K) \gtrsim \frac{\lambda_{\min}(H)^4}{d^4}.
\end{align*}

\paragraph{Simple case 2: $k$- symmetric (monomial) tensor $K$}
Suppose $K=\bv^{\otimes k}$ with $\bv \in \RR^{d^2}$ and $\norm{\bv}{}=1$. Then we have for any $i \in [k]$,
\begin{align*}
    \abs{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i} \otimes \paren{(r_n+r_{\star})(\bw)}^{\otimes i}} }&=\abs{\paren{\bv^{\top}\bT^{\star}\bw}^{k-i}\paren{\bv^{\top}(\br_{\star}+\br_n)\bw}^{i}}\\
    &\lesssim \abs{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i} \otimes \paren{(r_n+r_{\star})(\bw)}^{\otimes i}} }\\&=\abs{\paren{\bv^{\top}\bT^{\star}\bw}^{k-i}\paren{\bv^{\top}(\br_{\star}+\br_n)\bw}^{i}}\\
    &\lesssim\abs{\paren{\bv^{\top}\bT^{\star}\bw}^{k-i}\paren{\bv^{\top}\br_{\star}\bw}^{i}}+\abs{\paren{\bv^{\top}\bT^{\star}\bw}^{k-i}\paren{\bv^{\top}\br_{n}\bw}^{i}}.
\end{align*}
Thus, for any $i\in[k]$, we have
\begin{align*}
   &\quad\EE\brac{\abs{ K\paren{\paren{\bT^{\star}\bw}^{\otimes k-i} \otimes \paren{(r_n+r_{\star})(\bw)}^{\otimes i}} }^2 }\\
   &\lesssim \sqrt{\EE\brac{\paren{\bv^{\top}\bT^{\star}\bw}^{4(k-i)}}}\cdot \paren{\sqrt{\EE\brac{\paren{\bv^{\top}\br_{\star}\bw}^{4i}}}+\sqrt{\EE\brac{\paren{\bv^{\top}\br_{n}\bw}^{4i}}} }\\
   &\lesssim \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2}\frac{d^{2i}}{\lambda^{2i}_{\min}(H)} \cdot \paren{\frac{\norm{\br_{\star}}{op}^{2i}}{d^{2i}} +\frac{d^{2i}}{n^{i}}}
\end{align*}
On the other hand, the true signal 
\begin{align*}
    \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2}&=\EE\brac{\paren{\bv^{\top}\bT^{\star}\bw}^{2k}}\gtrsim \frac{\lambda^{2k}_{\min}(H)}{d^{2k}}\cdot 
\end{align*}
Thus, we only need to choose $n=Cd^4/\lambda_{\min}^2(H)$ and $d=\text{poly}(r)$ so that $\norm{\br_{\star}}{op}^2$ is small enough to ensure 
\begin{align*}
    \EE\brac{\paren{\Pi T_n(\bw)}^{\otimes 2k}}(K,K) \gtrsim \frac{\lambda_{\min}(H)^{2k}}{d^{2k}}.
\end{align*}


\paragraph{General case: $k$-symmetric tensor $K$}
Suppose $K=\sum_{i=1}^{p(r)}\lambda_i \bv_i^{\otimes k}$ with $\sum_{i=1}^{p(r)}\lambda_i^2=1$. \hengyu{$p(r)=r$ or $r^k$?} We can follow the proof above to derive a lower bound.

From this, we can directly obtain the following lemma:
\begin{lemma}
    Assuming $n\geq Cd^4/\lambda_{\min}^2(H)$ and $d\geq Cxxx$ for a sufficiently large constant C. Then for any symmetric $k$-tensor $K$ supported on the span of $\ba_1,\ba_2,\dots,\ba_r$, there exists $h(\bw)$ such that 
    \begin{align*}
        \EE\brac{h(\bw)(\bT_n(\bw)\cdot \bx)^{k}}=\langle K,\bx^{\otimes k} \rangle,
    \end{align*}
    and we have the bounds 
    \begin{align*}
        \EE\brac{h(\bw)^2}\lesssim \frac{d^{2k}}{\lambda_{\min}(H)^{2k}}\norm{K}{F}^2~~\text{and}~~ \abs{h(\bw)}  \lesssim \frac{d^{2k}}{\lambda_{\min}(H)^{2k}}\norm{K}{F}\abs{h(\bw)}^{k}.
    \end{align*}
\end{lemma}
\begin{proof}
    To realize the function, just let 
    \begin{align*}
        h(\bw)=\text{Vec}(K)^{\top}\text{Mat}\paren{\EE\brac{T_n(\bw)^{\otimes 2k}}}^{\dagger}\text{Vec}(\bT_{n}^{\otimes k}).
    \end{align*}
    By the discussion above, we have $\text{Vec}(K) \in \text{span}\paren{\EE\brac{T_n(\bw)^{\otimes 2k}}}$. Therefore, we can check that
    \begin{align*}
        &\quad\EE\brac{h(\bw)(\bT_n(\bw)\cdot \bx)^{k}}\\
        &=\EE\brac{\text{Vec}(K)^{\top}\text{Mat}\paren{\EE\brac{T_n(\bw)^{\otimes 2k}}}^{\dagger}\text{Vec}(\bT_{n}^{\otimes k})(\bT_n(\bw)\cdot \bx)^{k}}\\
        &=\langle K,\bx^{\otimes k} \rangle.
    \end{align*}
    For the bounds, we have
    \begin{align*}
        \EE\brac{h(\bw)^2}&=\text{Vec}(K)^{\top}\text{Mat}\paren{\EE\brac{T_n(\bw)^{\otimes 2k}}}^{\dagger}\text{Vec}(K)\\
        &\lesssim \frac{d^{2k}}{\lambda_{\min}(H)^{2k}}\norm{K}{F}^2,
    \end{align*}
    and
    \begin{align*}
        \abs{h(\bw)}=\abs{\text{Vec}(K)^{\top}\text{Mat}\paren{\EE\brac{T_n(\bw)^{\otimes 2k}}}^{\dagger}\text{Vec}(\bT_{n}^{\otimes k})}\lesssim \frac{d^{2k}}{\lambda_{\min}(H)^{2k}}\norm{K}{F}\abs{h(\bw)}^{k}
    \end{align*}
\end{proof}

This implies that we need to enlarge the learned feature by $d$ times ($\bT_n \rightarrow d\bT_n$), but accordingly, we need to show that $T_n(\bw)$ is bounded by $\cO\paren{\frac{1}{d}}$ with high probability.

\begin{lemma}
    With high probability, we have
    \begin{align*}
        \norm{T_n(\bw)}{}\lesssim \frac{\text{Log terms}}{d}
    \end{align*}
\end{lemma}
It suffices to prove that with high probability,
\begin{align*}
    \norm{T_n}{F}\lesssim 1.
\end{align*}
Recall that $T=\text{Vec}\paren{\EE\brac{f(\bx)x^{\otimes 4}}}$ \hengyu{Use hermite expansion?} Suppose that $f$ is even and $\EE\brac{f(\bx)}=\EE\brac{f(\bx)x^{\otimes 2}}=0$, we have $\norm{T}{F}^2 \lesssim \EE \brac{f(\bx)^2}=1$.
%Since $\lambda_{\min}(\bT^{\star})=\sqrt{2}\norm{H}{2}$, we can set $n\geq Cd^4\norm{H}{2}^2$ and $d \geq C  L^{4} r^{10}\log^8 d$ for sufficiently large $C$ so that 
%\begin{align}
%   \EE\brac{\delta(\bw)^2}\le \frac{1}{4} \EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2} \label{equ::delta expect bound}
%\end{align}
%Last, plugging \eqref{equ::delta expect bound} into \eqref{equ::lower bound T}, we have
%\begin{align*}
 %5   \EE\brac{\left\langle K, \paren{\Pi T_n(\bw)}^{\otimes k} \right\rangle^2} 
  %  &\geq \frac{1}{4}\EE\brac{\left\langle K, \paren{\bT^{\star}\bw}^{\otimes k} \right\rangle^2}\\
  %  &\gtrsim d^{-2k}\norm{\tilde K}{F}^2
%\end{align*}






\subsection{Extend to nonlinear case}
\hengyu{Challanges meet: I cannot do the trick to $r_{\star}$ as before since it is not linear.}
Comparison:
For an operator $\br: \RR^{d^2}\rightarrow \RR^{d^2}$, if we have $\norm{\br(\bw)}{2}\leq \epsilon$ for any unit vector $\bw$:
\begin{itemize}
    \item When $\br$ is linear and symmetric, we
    can write it as a matrix $\br \in \RR^{d^2\times d^2}$ with $\norm{\br}{op}\le \epsilon$. Then for a unit vector $\bv$,  $\EE\brac{\langle \bv, \br(\bw)\rangle^2}=\frac{\norm{\br \bv}{F}^2}{d^2}\le \frac{\epsilon^2}{d^2}$. Here $\bw \sim \frac{1}{d}\cN(0,\bI_{d^2})$.
    \item If $\br$ is nonlinear, we only have $\EE\brac{\langle \bv,\br(\bw)\rangle^2}=\EE\brac{\norm{\br(\bw)}{2}^2\norm{\bv}{2}^2}\le {\epsilon^2}$. \hengyu{Maybe we need to prove $\br(\bw)$ is also approximately gaussian so it has only an averaged correlation with $\bv$, i.e. $\frac{1}{d^2}$}

\end{itemize}
Some inspiring examples:
\begin{itemize}
    \item When $r=1$, $f(\bx)=(x^{\top}Ax)^2-1$ and another $W\in \RR^{d\times d}$, we have
    \begin{align*}
        \EE\brac{f(\bx)\langle W,\bx\bx^{\top}\rangle \bx\bx^{\top}}=8A^{\top}WA+16A^{\top}AW+4\langle W,A\rangle A,
    \end{align*}
    Here the error term is $r(W)=8A^{\top}WA+16A^{\top}AW$, which satisfies $$\norm{r(W)}{F}\lesssim \frac{1}{d}\norm{W}{F}.$$
    This implies we always get at least $\cO(\frac{1}{d})$ error in terms of Frob-norm.
\end{itemize}

Hope to check:
    \begin{itemize}
        \item $\norm{\EE_{x}\brac{f(\bx)\text{He}_{k}\paren{x^{\top}Wx}\bx\bx^{\top}}}{F} =\cO(\frac{1}{d^2})$ for $k\geq 2.$
    \end{itemize}

\begin{lemma}
    We suppose the function $g:\RR^{r}\rightarrow \RR$ satisfies $\EE_{\bz \sim \cN(0,\bI_r)}\brac{g(\bz)}=0$, $\EE\brac{\nabla g(\bz)}=\mathbf{0}_{r}$ and $\EE\brac{g(\bz)^2}=1$. For any standard multivariate normal variable $\bz\sim \cN(0,\bI_r)$ and $\tilde z_1, \tilde z_2\sim \cN(0,1)$ satisfying $\norm{\text{Cov}(\bz,\tilde z_1)}{2} \le \epsilon<1$, we have
    \begin{align*}
        \abs{\EE_{\bz,\tilde z_1,\tilde z_2}\brac{g(\bz) \He_{k}(\tilde  z_1)\tilde z_2}}\le \epsilon^{k}\sqrt{k!}+\mathbf{1}_{k\geq 3}k\epsilon^{k-1}\sqrt{2(k-1)!}.
    \end{align*}
\end{lemma}
This lemma implies that if $\epsilon \le \cO(\sqrt{r}/d)$, we have the high order terms $(k\geq 2)$ bounded by $\cO(r/d^2)$
\begin{proof}
    We first consider the case $\tilde z_2=z_i$ for $i \in [r]$. W.L.O.G., we assume $i=1$. Then we decompose $\tilde z_1$ as
    \begin{align*}
        \tilde z_1=\gamma\cdot \bc^{\top}\bz + \tilde \gamma z_{r+1},
    \end{align*}
    where $\norm{\bc}{}=1$, $\gamma\geq 0$ and $ z_{r+1}$ is another standard normal variable independent of any $z_i$, $i\in[r]$. By our assumptions on $\tilde z_1$, we directly have $\gamma\le \epsilon$ and $\gamma^2+\tilde \gamma^2=1$. By Taylor expansion, we have
    \begin{align*}
        \He_k(\tilde z_1)=\sum_{i=0}^{k}C_{k}^{i}\He_{k-i}\paren{\gamma\cdot \bc^{\top}\bz}\paren{\tilde \gamma z_{r+1}}^{i}.
    \end{align*}
    Since $\EE\brac{z_{r+1}^{i}}=(i-1)!!$ if $i$ is even and $0$ if odd, we have
    \begin{align*}
        \EE_{\bz,\tilde z_1}\brac{g(\bz) \He_{k}(\tilde  z_1)z_1}=\sum_{i=0}^{\lfloor{\frac{k}{2}}\rfloor}C_{k}^{2i}(2i-1)!!\tilde \gamma^{2i}\EE_{\bz}\brac{g(\bz)\He_{k-2i}\paren{\gamma\cdot \bc^{\top}\bz}z_1}.
    \end{align*}
    Furthermore, we expand $\He_{k-2i}\paren{\gamma\cdot \bc^{\top}\bz}$ as
    \begin{align*}
        \He_{k-2i}\paren{\gamma\cdot \bc^{\top}\bz}=\sum_{j=0}^{\lfloor\frac{k}{2}-i\rfloor}\gamma^{k-2i-2j}(\gamma^2-1)^{j}C_{k-2i}^{2j}(2j-1)!!\He_{k-2i-2j}(\bc^{\top}\bz),
    \end{align*}
    which gives rise to 
    \begin{align}\label{equ::Hek}
        \EE_{\bz,\tilde z_1}\brac{g(\bz) \He_{k}(\tilde  z_1)z_1}=\sum_{m=0}^{\lfloor{\frac{k}{2}}\rfloor}c_m\gamma^{k-2m}(1-\gamma^2)^{m}\EE_{\bz}\brac{g(\bz)\He_{k-2m}\paren{ \bc^{\top}\bz}z_1},
    \end{align}
    where $\set{c_m}$ is a set of constants satisfying 
    \begin{align*}
        c_m&=\sum_{j=0}^{m}(-1)^{m-j}C^{2(m-j)}_{k}(2(m-j)-1)!! C_{k-2(m-j)}^{2j}(2j-1)!! \\
        &=\sum_{j=0}^{m} (-1)^{m-j}\frac{k!}{2^{m}(m-j)!j!(k-2m)!}\\
        &=\sum_{j=0}^{m} (-1)^{m-j}\frac{m!}{ (m-j)!j!}  \frac{k!}{2^m m!(k-2m)! }\\
        &=\mathbf{1}_{m=0}.
    \end{align*}
    Moreover, we have 
    \begin{align*}
        \EE_{\bz}\brac{g(\bz)\He_{k-2m}\paren{ \bc^{\top}\bz}z_1}&=\EE_{\bz}\brac{\langle\nabla^{k-2m}\brac{g(\bz)z_1},\bc^{\otimes k-2m}\rangle}\\
        &=\EE_{\bz}\brac{z_1\langle\nabla^{k-2m}g(\bz),\bc^{\otimes k-2m}\rangle\rangle}\\
        &\quad+\EE_{\bz}\brac{(k-2m)\langle\nabla^{k-2m-1}g(\bz) \otimes \be_1,\bc^{\otimes k-2m}}\\
        &=\EE_{\bz}\brac{\langle\nabla^{k-2m+1}g(\bz),\be_1\otimes \bc^{\otimes k-2m}\rangle\rangle}\\
        &\quad+(k-2m)\EE_{\bz}\brac{\langle\nabla^{k-2m-1}g(\bz) \otimes \be_1,\bc^{\otimes k-2m}}.
    \end{align*}
    Plugging into \eqref{equ::Hek} gives rise to
    \begin{align*}
        \EE_{\bz,\tilde z_1}\brac{g(\bz) \He_{k}(\tilde  z_1)z_1}&=\gamma^{k}\EE_{\bz}\brac{g(\bz)\He_{k}(\bc^{\top}\bz)z_1}\\
        &=\gamma^{k}\EE_{\bz}\brac{\langle\nabla^{k+1}g(\bz),\be_1\otimes \bc^{\otimes k}\rangle\rangle}\\
        &\quad+k\gamma^{k}\EE_{\bz}\brac{\langle\nabla^{k-1}g(\bz) \otimes \be_1,\bc^{\otimes k}}.
    \end{align*}

    Now we consider the case $\tilde z_2=z_{r+1}$. Then we similarly have
    \begin{align*}
        \EE_{\bz,\tilde z_1,\tilde z_2}\brac{g(\bz) \He_{k}(\tilde  z_1)\tilde z_2}&=\EE_{\bz, z_{r+1}}\brac{g(\bz) \He_{k}(\gamma \bc^{\top}\bz+\tilde \gamma ) z_{r+1}}\\
        &=\tilde \gamma k\EE_{\bz, z_{r+1}}\brac{g(\bz) \He_{k-1}(\gamma \bc^{\top}\bz+\tilde \gamma z_{r+1})}\\
        &=k\tilde \gamma \gamma^{k-1} \EE\brac{g(\bz)\He_{k-1}(\bc^{\top}\bz)}\\
        &=k\tilde \gamma \gamma^{k-1} \EE\brac{\langle\nabla^{k-1}g(\bz),\bc^{\otimes k-1}\rangle}.
    \end{align*}
    Thus, for $k=1$ and any $\tilde z_2 \sim \cN(0,1)$, by $\EE g(\bz)=0$ we have
    \begin{align*}
         \abs{\EE_{\bz,\tilde z_1,\tilde z_2}\brac{g(\bz) \He_{k}(\tilde  z_1)\tilde z_2}}\le \gamma \norm{\EE\brac{\nabla^{2}g(\bz)}}{F}\le \sqrt{2}\gamma.
    \end{align*}
    For $k\geq 2$, we have
    \begin{align*}
        \abs{\EE_{\bz,\tilde z_1,\tilde z_2}\brac{g(\bz) \He_{k}(\tilde  z_1)\tilde z_2}}&\le \gamma^{k}\norm{\EE\brac{\nabla^{k+1}g(\bz)}}{F}+k\gamma^{k-1}(\gamma+\tilde \gamma)\norm{\EE\brac{\nabla^{k-1}g(\bz)}}{F}\\
        &\le \gamma^{k}\sqrt{k!}+\mathbf{1}_{k\geq 3}k\gamma^{k-1}\sqrt{2(k-1)!},
    \end{align*}
       % \le \sum_{m=0}^{\lfloor\frac{k}{2}\rfloor}\gamma^{k}2^{k-2m}\frac{k!}{(k-m)!}\paren{\norm{C_{k-2m+1}}{F}+(k-2m)\norm{C_{k-2m-1}}{F}}\\
       % &\lesssim \gamma^{k}2^{2k}k!,
    where we invoke $\norm{\EE\brac{\nabla^{k}g(\bz)}}{F}\le \sqrt{j!}$ in the inequality. Plugging $\gamma \le \epsilon$ concludes our proof.
\end{proof}

==> deprecated/deprecated_concentration.tex <==
\subsubsection{Concentration on the features}
For any $\bA\in\RR^{d\times d}$ such that $\tr(\bA)=0$, we have
\begin{align*}
    \EE_{\bv}\brac{(\bv^{\top}\bA\bv)(\bv\bv^{\top}-\bI)}=b_2\bA,
\end{align*}
where $b_2=\frac{2d}{d+2}$. Let's consider its concentration on $m_2$:
\begin{lemma}\label{lemma:: reconstruct A}
    Given any symmetric matrix $\bA \in \RR^{d \times d}$ such that $\tr(A)=0$ and $\tau \geq 0$, we have 
    \begin{align*}
         &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}(\bv_i^{\top}\bA\bv_i)(\bv_i\bv_i^{\top}-\bI_d)-b_2\bA}{2}\geq \tau}\\
    &\le 2d\exp\paren{-\frac{m_2\tau^2/2}{{2d(\norm{\bA}{2}^2\vee 1)}+(d^2+2)\norm{\bA}{2}\tau/3}}.
    \end{align*}
\end{lemma}
\begin{proof}[Proof of \cref{lemma:: reconstruct A}]
Denote the random matrix $\bZ_i=(\bv_i^{\top}\bA\bv_i)(\bv_i\bv_i^{\top}-\bI_d)-b_2\bA$. Then we have $\EE\brac{\bZ_i}=\bzero_{d\times d}$, and 
\begin{align*}
    \norm{\bZ_i}{2}&\le \bv_i^{\top}\bA\bv_i\norm{\bv_i\bv_i^{\top}-\bI_d}{2}+b_2\norm{\bA}{2}\\
    &\le \norm{\bA}{2}\norm{\bv_i}{2}^2\norm{\bv_i\bv_i^{\top}-\bI_d}{F}+b_2\norm{\bA}{2}\\
    &\le (d^2+b_2)\norm{\bA}{2}\\
    &\le (d^2+2)\norm{\bA}{2}
    ,\\
    \norm{\EE\brac{\bZ_i\bZ_i^{\top}}}{2}&=\norm{\EE\brac{(\bv_i^{\top}\bA\bv_i)^2(\bv_i\bv_i^{\top}-\bI_d)^2}-b_2^2\bA^2}{2}\\
    &=\norm{\EE\brac{(\bv_i^{\top}\bA\bv_i)^2((d-2)\bv_i\bv_i^{\top}+\bI_d)}-b_2^2\bA^2}{2}\\
    &=\norm{\frac{(d-2)d^2}{(d+2)(d+4)}\bA^2+(d-1)\bI_d-b_2^2\bA^2}{2}\\
    &\le 2d(\norm{\bA}{2}^2\vee 1).
\end{align*}
Thus, by matrix Berstein inequality, we have
\begin{align*}
    &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}(\bv_i^{\top}\bA\bv_i)(\bv_i\bv_i^{\top}-\bI_d)-b_2\bA}{2}\geq \tau}\\
    &= \Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bZ_i}{2}\geq \tau}\\
    &\le 2d\exp\paren{-\frac{m_2\tau^2/2}{{2d(\norm{\bA}{2}^2\vee 1)}+(d^2+2)\norm{\bA}{2}\tau/3}}.
\end{align*}
The proof is complete.
\end{proof}





% \begin{proof}
%     Considering the scaled case $\frac{1}{m_2}P^{\top}\sigma_2(V^{\top}x)=\frac{1}{m_2}\sum_{i=1}^{m_2}\sigma_2(v_i^{\top}x)\bp(\bv_i) \rightarrow \EE_v \brac{\sigma_2(v^{\top}x)\bp(\bv)} \in \RR^{r}$. Denote $\gamma(v)=\sigma_2(v^{\top}x)\bp(\bv)$, then $\norm{\gamma(v)}{}^{2}\le\sum_{k=1}^{r}(v^{\top}Av)^2\le rd$ for any $v\in \mathbb{S}^{d-1}(\sqrt{d})$. Here we assume $\abs{\sigma_2(v^{\top}x)}\le 1$. Moreover, we have
% \begin{align*}
%     \EE_{v}\brac{\norm{\gamma(v)}{}^2}\le \EE_v\brac{\sum_{k=1}^{r}(v^{\top}Av)^2}=r. 
% \end{align*}
% Again by Matrix-Bernstein Inequality, we have
% \begin{align*}
%     &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\sigma_2(v_i^{\top}x)\bp(\bv_i)- \EE_v \brac{\sigma_2(v^{\top}x)\bp(\bv)}}{}\geq \sqrt{\frac{r}{m_2}\log \tau} }\\
%     &\le(r+1)\exp\paren{\frac{-\frac{r}{2m_2}\log\tau}{\frac{r}{m_2}+\frac{\sqrt{rd}}{3m_2}\sqrt{\frac{r}{m_2}\log \tau}}}\\
%     &=(r+1)\exp\paren{\frac{-\frac{1}{2}\log \tau}{1+\frac{1}{3}\sqrt{\frac{d}{m_2}\log\tau}}}.
% \end{align*}
% Thus, only taking $\log\tau =\cO(\log \epsilon^{-1})$ is needed for an $r\epsilon$ error.

% Another choice of $m_2$ is $m_2=rd^2$ \hengyu{check}, which gives a tighter concentration with length of the confidence interval independent of $r$.
% \end{proof}



Let $\bp(\bv)=[\bv^{\top}\bA_r\bv]^{\top}\in\RR^{r}$, which is the target features. Since $\EE\brac{\bp(\bv)}=\mathbf{0}$ and $\Var\brac{\bp(\bv)}=\bI$, we have the following concentration lemma:
\begin{lemma}
    For any $\tau \geq 0$, we have 
    \begin{align*}
           &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bp(\bv_i)\bp(\bv_i)^{\top}-\bI_{r}}{2}\geq \tau}\\
     &\le 2B(d,2)\exp\paren{\frac{-m_2\tau^2/2}{(B(d,2 )-1)+B(d,2)\cdot\tau/3}}.
    \end{align*}
\end{lemma}
\begin{proof}
    Since $\tr(\bA_i)=0$ for all $i\in[r]$, $\bv^{\top}\bA_i\bv$ can be decomposed into the sum of quadratic spherical harmonics. Suppose $\bv^{\top}\bA_i\bv=\bu_i^{\top}\bY_{2}(\bv)$ where $\bu_i\in\RR^{m_2}$. Then by Assumption \ref{assump::features} we know that $\{\bu_i\}_{i=1}^{r}$ are $r$ orthogonal unit vectors. Denoting $\bU=[\bu_1,\bu_2,\cdots,\bu_r]\in \RR^{m_2\times r}$, we can write $\bp(\bv)=\bU^{\top}\bY_2(\bv)$. Thus, we have 
    \begin{align*}
        \norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bp(\bv_i)\bp(\bv_i)^{\top}-\bI_{r}}{2}&=\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\paren{\bU^{\top}\bY_2(\bv)\bY_2(\bv)^{\top}\bU-\bI_r}}{2}\\
        &=\norm{\bU^{\top}\cdot\frac{1}{m_2}\sum_{i=1}^{m_2}\paren{\bA_{2,2}(\bv_i)-\bI_{B(d,2)}}\cdot\bU}{2}\\
        &=\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bA_{2,2}(\bv_i)-\bI_{B(d,2)}}{2}
        \end{align*}
 Here we invoke the fact that $\bU$ has unit and orthogonal columns in the last equality. Thus, by Corollary \ref{coro::spherical product} with $k=2$, we have
 \begin{align*}
     &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bp(\bv_i)\bp(\bv_i)^{\top}-\bI_{r}}{2}\geq \tau}\\
     &\le 2B(d,2)\exp\paren{\frac{-m_2\tau^2/2}{(B(d,2 )-1)+B(d,2)\cdot\tau/3}}
 \end{align*}
 The proof is complete.
\end{proof}


% \begin{proof}

% Let $\bp(\bv)=[\bv^{\top}\bA_r\bv]_{k\in [r]} \in \RR^{r}$, then we have $\frac{1}{m_2}\bP^{\top}\bP=\frac{1}{m_2}\sum_{i=1}^{m_2}\bp(\bv_i)\bp(\bv_i)^{\top}$. Since we have
% \begin{align*}
%     \EE_{v}\brac{\bp(\bv)\bp(\bv)^{\top}\bp(\bv)\bp(\bv)^{\top}}=\EE_{v}\brac{\brac{\sum_{k=1}^{r}(v^{\top}\bA_kv)^2}\bp(\bv)\bp(\bv)^{\top}}=(r+2+o(1))I_k.
% \end{align*}
% \hengyu{check}
% Moreover, we have $\norm{\bp(\bv)\bp(\bv)^{\top}}{}=\norm{\bp(\bv)}{2}^2=\sum_{k=1}^{r}(v^{\top}\bA_kv)^2\le r\norm{\bA_k}{}^2 \norm{v}{2}^4\lesssim rd$ with probability 1. 
% Thus, by Matrix-Bernstein Inequality, we have
% \begin{align*}
%     \Pr\brac{\norm{\frac{1}{m_2}\bP^{\top}\bP-I_r}{}\geq \sqrt{\frac{r}{m_2} \log \tau }}&=2r\exp\paren{\frac{-\frac{r}{2m_2} \log \tau }{\frac{r+\cO(1)}{m_2}+\frac{rd}{3m_2}\sqrt{\frac{r}{m_2} \log \tau }}}\\
%     &=2r\exp\paren{\frac{-\frac{1}{2}\log \tau}{1+o(1)+\frac{1}{3}\sqrt{\frac{rd^2}{m_2}\log \tau}}}.
% \end{align*}


% When $m_2=d^2$, this becomes
% \begin{align*}
%     \Pr\brac{\norm{\frac{1}{m_2}\bP^{\top}\bP-I_r}{}\geq \frac{1}{d}\sqrt{r \log \tau }}&=2r\exp\paren{\frac{-\frac{r}{2d^2} \log \tau }{\frac{r+\cO(1)}{d^2}+\frac{rd}{3d^2}\sqrt{\frac{r}{d^2} \log \tau }}}\\
%     &\le 2r\exp\paren{\frac{-\log \tau /2}{{1+o(1)}+\sqrt{r\log \tau}/3}}.
% \end{align*}
% Taking $\log\tau=4r(\log \epsilon)^2/9+2\log \epsilon^{-1}$ gives
% \begin{align*}
%     2r\exp\paren{\frac{-\log \tau /2}{{1+o(1)}+\sqrt{r\log \tau}/3}}\le 2r\epsilon.
% \end{align*}
% Thus, we have
% \begin{align*}
%     \Pr\brac{\norm{\frac{1}{m_2}\bP^{\top}\bP-I_r}{}\geq \frac{2r\log \epsilon^{-1}\sqrt{1+9/(2r\log \epsilon^{-1})}}{3d}}&\le 2r\epsilon.
% \end{align*}
% \end{proof}

Next, let's focus on the concentration of $\EE_{\bv}\brac{(\bv^{\top}\bA_k\bv)Q_2(\bv^{\top}\bx)}$.

\begin{lemma}\label{lemma:: concentration vtAvQ2x}
    Given $\tau\geq 0$, we have 
    \begin{align*}
        &\quad\Pr\brac{\abs{\frac{1}{m_2}\sum_{i=1}^{m_2}(\bv_i^{\top}\bA\bv_i)Q_2(\bv_i^{\top}\bx)-\frac{1}{B(d,2)}\bx^{\top}\bA\bx}\geq \tau}\\& \le 2B(d,2)\exp\paren{\frac{-m_2\tau^2/2}{1+\sqrt{B(d,2)}\cdot\tau/3}}
    \end{align*}
\end{lemma}
for any matrix $\bA$ such that $\EE\brac{\bv^{\top}\bA\bv}=0$  and $\EE\brac{(\bv^{\top}\bA\bv)^2}=1$.
Here $B(d,2)=\frac{2}{(d+2)(d-1)}$. 
\begin{proof}[Proof of Lemma \ref{lemma:: concentration vtAvQ2x}]
    Since $\EE\brac{\bv^{\top}\bA\bv}=0$  and $\EE\brac{(\bv^{\top}\bA\bv)^2}=1$, we know $\tr(\bA)=0$ and $\norm{\bA}{F}^2=b_2^{-1}=\frac{d+2}{2d}.$ Thus, $\bv^{\top}\bA\bv$ can be decomposed into the sum of quadratic spherical harmonics. Suppose $\bv^{\top}\bA\bv=\bu^{\top}\bY_{2}(\bv)$ where $\bu\in\RR^{m_2}$ and $\norm{\bu}{2}=1$. 
    % Suppose $\bA=\sum_{j=1}^{d}\lambda_j\bu_j\bu_j^{\top}$, where $\set{\bu_j}_{j=1}^{d}$ are unit vectors that are orthogonal to each other. Then we have $\sum_{j=1}^{d}\lambda_j=0$ and $\sum_{j=1}^{d}\lambda_j^{2}=\frac{d+2}{2d}.$ 
    Then, by the properties of spherical harmonics and Gegenbauer polynomials, for any $i \in[m_2]$ and $\bx\in \RR^{d}$, we have 
    \begin{align*}
    (\bv^{\top}\bA\bv)Q_2(\bv^{\top}\bx)&=\bu^{\top}\bY_{2}(\bv)\cdot\frac{1}{B(d,2)}\sum_{j=1}^{B(d,2)}Y_{2,j}(\bv)Y_{2,j}(\bx)\\
    &=\frac{1}{B(d,2)}\bu^{\top}\bA_{2,2}(\bv)\bY_2(\bx)
    \end{align*}
    Since $\EE_{\bv}\brac{\bA_{2,2}(\bv)}=\bI_{B(d,2)}$, we have $$\EE\brac{(\bv^{\top}\bA\bv)Q_2(\bv^{\top}\bx)}=\frac{1}{B(d,2)}\bu^{\top}\bY_2(\bx)=\frac{1}{B(d,2)}\bx^{\top}\bA\bx.$$
    Thus, for any $\tau \geq 0$, we obtain that
    \begin{align*}
        &\quad\Pr\brac{\abs{\frac{1}{m_2}\sum_{i=1}^{m_2}(\bv_i^{\top}\bA\bv_i)Q_2(\bv_i^{\top}\bx)-\frac{1}{B(d,2)}\bx^{\top}\bA\bx}\geq \tau}\\
        &=\Pr\brac{\abs{\frac{1}{B(d,2)}\bu^{\top}\paren{\frac{1}{m_2}\sum_{i=1}^{m_2}\paren{\bA_{2,2}(\bv_i)-\bI_{B(d,2)}}}\bY_2(\bx)}\geq \tau}\\
        &\le \Pr\brac{\frac{1}{B(d,2)}\norm{\bu}{2}\norm{\paren{\frac{1}{m_2}\sum_{i=1}^{m_2}\paren{\bA_{2,2}(\bv_i)-\bI_{B(d,2)}}}}{2}\norm{\bY_2(\bx)}{2}\geq \tau}\\
        &=\Pr\brac{\norm{\paren{\frac{1}{m_2}\sum_{i=1}^{m_2}\paren{\bA_{2,2}(\bv_i)-\bI_{B(d,2)}}}}{2}\geq {\sqrt{B(d,2)}}{\tau}}\\
        &\le 2B(d,2)\exp\paren{\frac{-m_2B(d,2)\tau^2/2}{(B(d,2 )-1)+{B(d,2)}^{3/2}\cdot\tau/3}}\\
        &\le 2B(d,2)\exp\paren{\frac{-m_2\tau^2/2}{1+\sqrt{B(d,2)}\cdot\tau/3}}.
    \end{align*}
    In the second inequality we invoke Corollary \ref{coro::spherical product} with $k=2$. The proof is complete.
\end{proof}

Following the proof above, we directly have the following lemma.
\begin{corollary}
    
\label{coro:: concentration vtAvQkx}
    Given $\tau\geq 0$ and any integer $k>2$, we have 
    \begin{align*}
        \Pr\brac{\abs{\frac{1}{m_2}\sum_{i=1}^{m_2}(\bv_i^{\top}\bA\bv_i)Q_k(\bv_i^{\top}\bx)}\geq \tau}& \le 2B(d,k)\exp\paren{\frac{-m_2\tau^2/2}{1+\sqrt{B(d,k)}\cdot\tau/3}},
    \end{align*}
     for any matrix $\bA$ such that $\EE\brac{\bv^{\top}\bA\bv}=0$  and $\EE\brac{(\bv^{\top}\bA\bv)^2}=1$.
\end{corollary}



\begin{lemma}\label{lemma::concentration of spherical product}
    Let $\bY_{k}(\bx)=[Y_{k,1}(\bx),\cdots,Y_{k,B(d,k)}(\bx)]^{\top}\in\RR^{B(d,k)}$ be the vector of all degree-$k$ spherical harmonics and let $\bA_{k_1,k_2}(\bx)=\bY_{k_1}(\bx)\bY_{k_2}(\bx)^{\top} \in \RR^{B(d,k_1) \times B(d,k_2) }$ for any positive integers $k_1< k_2$. Then for all $\tau \geq 0$, we have 
    \begin{align*}
       &\quad \Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bA_{k_1,k_2}(\bv_i)}{2}\geq \tau } \\
        &\le(B(d,k_1)+B(d,k_2)) \exp\paren{\frac{-m_2\tau^2/2}{B(d,k_2 )+\sqrt{B(d,k_1)B(d,k_2)}\cdot\tau/3}} .
    \end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma::concentration of spherical product}]
We know that $\EE_{\bv}\brac{\bA_{k_1,k_2}(\bv)}=\bzero_{B(d,k_1)\times B(d,k_2)}$. Note that for any $\bv \in \SS^{d-1}(\sqrt d)$, we have 
\begin{align*}
    \norm{\bA_{k_1,k_2}(\bv)}{2}&=\norm{\bY_{k_1}(\bv)}{2}\norm{\bY_{k_2}(\bv)}{2}\\
    &=\sqrt{\sum_{i=1}^{B(d,k_1)}Y_{k_1,i}^2(\bv)\sum_{i=1}^{B(d,k_2)}Y_{k_2,i}^2(\bv)}\\
    &=\sqrt{B(d,k_1)Q_{k_1}^{}(d)B(d,k_2)Q_{k_2}^{}(d)}\\
    &=\sqrt{B(d,k_1)B(d,k_2)},
\end{align*}
and we can further obtain that
\begin{align*}
    \EE_{\bv}\brac{\bA_{k_1,k_2}(\bv)^{\top}\bA_{k_1,k_2}(\bv)}&=\EE_{\bv}\brac{\bY_{k_2}(\bv)\bY_{k_2}(\bv)^{\top}\norm{\bY_{k_1}^2(\bv)}{2}^2}\\
    &=B(d,k_1)\bI_{B(d,k_2)}
\end{align*}
and similarly
\begin{align*}
    \EE_{\bv}\brac{\bA_{k_1,k_2}(\bv)\bA_{k_1,k_2}^{\top}(\bv)}&=\EE_{\bv}\brac{\bY_{k_1}(\bv)\bY_{k_1}(\bv)^{\top}\norm{\bY_{k_2}^2(\bv)}{2}^2}\\
    &=B(d,k_2)\bI_{B(d,k_1)}.
\end{align*}
Thus, by matrix Bernstein inequality, we have
\begin{align*}
   &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bA_{k_1,k_2}(\bv_i)}{2}\geq \tau } \\&\le (B(d,k_1)+B(d,k_2)) \exp\paren{\frac{-\tau^2/2}{{B(d,k_1\vee k_2 )}/{m_2}+\sqrt{B(d,k_1)B(d,k_2)}\cdot\tau/(3m_2)}} \\
   &=(B(d,k_1)+B(d,k_2)) \exp\paren{\frac{-m_2\tau^2/2}{B(d,k_2 )+\sqrt{B(d,k_1)B(d,k_2)}\cdot\tau/3}}
\end{align*}
The proof is complete.
\end{proof}
By the same proof, we have the following corollary with the case $k_1=k_2$:
\begin{corollary}\label{coro::spherical product}
    For any positive integer $k$ and $\tau \geq 0$, we have 
    \begin{align*}
       &\quad \Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bA_{k,k}(\bv_i)-\bI_{B(d,k)}}{2}\geq \tau}\\
        &\le 2B(d,k)\exp\paren{\frac{-m_2\tau^2/2}{(B(d,k )-1)+B(d,k)\cdot\tau/3}}.
    \end{align*}
\end{corollary}
\begin{proof}[Proof of \cref{coro::spherical product}]
By the properties of spherical harmonics and following the proof of \cref{lemma::concentration of spherical product}, we have 
\begin{align*}
    &\hspace{7em}\EE_{\bv}\brac{\bA_{k,k}(\bv)}=\bI_{B(d,k)},~~~\norm{\bA_{k,k}}{2}=B(d,k),~~~\text{and}\\
    &\EE_{\bv}\brac{\bA_{k,k}(\bv)\bA_{k,k}(\bv)^{\top}-\bI_{B(d,k)}^2}=\EE_{\bv}\brac{\bA_{k,k}(\bv)^{\top}\bA_{k,k}(\bv)-\bI_{B(d,k)}^2}=(B(d,k)-1)\bI_{B(d,k)}.
\end{align*}
Thus, by matrix Bernstein inequality, we have
\begin{align*}
   &\quad\Pr\brac{\norm{\frac{1}{m_2}\sum_{i=1}^{m_2}\bA_{k,k}(\bv_i)-\bI_{B(d,k)}}{2}\geq \tau } \\&\le (B(d,k)+B(d,k)) \exp\paren{\frac{-\tau^2/2}{{(B(d,k )-1)}/{m_2}+B(d,k)\cdot\tau/(3m_2)}} \\
   &=2B(d,k) \exp\paren{\frac{-m_2\tau^2/2}{(B(d,k )-1)+B(d,k)\cdot\tau/3}}.
\end{align*}
    The proof is complete.
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preview/hengyu-learning_multiple_nonlinear_features_large.tex <==
%\def\usebigfont{1}
\input{iclr2025_conference}
